Finding a Hidden Edge

We consider the problem of finding an edge in a hidden undirected graph $G = (V, E)$ with $n$ vertices, in a model where we only allowed queries that ask whether or not a subset of vertices contains an edge. We study the non-adaptive model and show that while in the deterministic model the optimal algorithm requires $\binom{n}{2}$ queries (i.e., querying for any possible edge separately), in the randomized model $\tilde{\Theta}(n)$ queries are sufficient (and needed) in order to find an edge. In addition, we study the query complexity for specific families of graphs, including Stars, Cliques, and Matchings, for both the randomized and deterministic models. Lastly, for general graphs, we show a trade-off between the query complexity and the number of rounds, $r$, made by an adaptive algorithm. We present two algorithms with $O(rn^{2/r})$ and $\tilde{O}(rn^{1/r})$ sample complexity for the deterministic and randomized models, respectively.

==> lipics-v2021-sample-article.tex <==
%\documentclass[a4paper,UKenglish,cleveref, autoref,anonymous, thm-restate]{lipics-v2021}
%This is a template for producing LIPIcs articles. 
%See lipics-v2021-authors-guidelines.pdf for further information.
%for A4 paper format use option "a4paper", for US-letter use option "letterpaper"
%for british hyphenation rules use option "UKenglish", for american hyphenation rules use option "USenglish"
%for section-numbered lemmas etc., use "numberwithinsect"
%for enabling cleveref support, use "cleveref"
%for enabling autoref support, use "autoref"
%for anonymousing the authors (e.g. for double-blind review), add "anonymous"
%for enabling thm-restate support, use "thm-restate"
%for enabling a two-column layout for the author/affilation part (only applicable for > 6 authors), use "authorcolumns"
%for producing a PDF according the PDF/A standard, add "pdfa"

\pdfoutput=1 %uncomment to ensure pdflatex processing (mandatatory e.g. to submit to arXiv)
\hideLIPIcs  %uncomment to remove references to LIPIcs series (logo, DOI, ...), e.g. when preparing a pre-final version to be uploaded to arXiv or another public repository

%\graphicspath{{./graphics/}}%helpful if your graphic files are in another directory

\bibliographystyle{plainurl}% the mandatory bibstyle

\title{Finding a Hidden Edge} %TODO Please add

%\titlerunning{Dummy short title} %TODO optional, please use if title is longer than one line

\author{Ron Kupfer}{Harvard University}{ron.kupfer@mail.huji.ac.il}{}{(Optional) author-specific funding acknowledgements}%TODO mandatory, please use full name; only 1 author per \author macro; first two parameters are mandatory, other parameters can be empty. Please provide at least the name of the affiliation and the country. The full address is optional. Use additional curly braces to indicate the correct name splitting when the last name consists of multiple name parts.

\author{Noam Nisan}{Hebrew University}{noam@cs.huji.av.il}{}{[funding]}

\authorrunning{R. Kupfer and N. Nisan} %TODO mandatory. First: Use abbreviated first/middle names. Second (only in severe cases): Use first author plus 'et al.'

\Copyright{Ron Kupfer and Noam Nisan} %TODO mandatory, please use full first names. LIPIcs license is "CC-BY";  http://creativecommons.org/licenses/by/3.0/

\ccsdesc{Theory of computation}
%\ccsdesc[100]{\textcolor{red}{Replace ccsdesc macro with valid one}} %TODO mandatory: Please choose ACM 2012 classifications from https://dl.acm.org/ccs/ccs_flat.cfm 

\keywords{query complexity, non-adaptive algorithms, randomized vs. deterministic} %TODO mandatory; please add comma-separated list of keywords

\category{} %optional, e.g. invited paper

\relatedversion{} %optional, e.g. full version hosted on arXiv, HAL, or other respository/website
%\relatedversiondetails[linktext={opt. text shown instead of the URL}, cite=DBLP:books/mk/GrayR93]{Classification (e.g. Full Version, Extended Version, Previous Version}{URL to related version} %linktext and cite are optional

%\supplement{}%optional, e.g. related research data, source code, ... hosted on a repository like zenodo, figshare, GitHub, ...
%\supplementdetails[linktext={opt. text shown instead of the URL}, cite=DBLP:books/mk/GrayR93, subcategory={Description, Subcategory}, swhid={Software Heritage Identifier}]{General Classification (e.g. Software, Dataset, Model, ...)}{URL to related version} %linktext, cite, and subcategory are optional

%\funding{(Optional) general funding statement \dots}%optional, to capture a funding statement, which applies to all authors. Please enter author specific funding statements as fifth argument of the \author macro.

%\acknowledgements{I want to thank \dots}%optional

%\nolinenumbers %uncomment to disable line numbering
\usepackage{thm-restate}
\declaretheorem[name=Theorem, sibling=theorem]{rThm}
\declaretheorem[name=Lemma, sibling=lemma]{rLem}
\declaretheorem[name=Corollary, sibling=corollary]{rCor}
\declaretheorem[name=Proposition, sibling=proposition]{rPro}


\newcommand{\ron}[1]{{\color{red} Ron: #1}}
\newcommand{\ronedit}[1]{{\color{green}#1}}
\newcommand{\stam}[1]{}
\newcommand{\TBD}[1]{{\color{red}TBD: #1}}

\newcommand{\CC}[1]{\capitalisewords{#1}}
\newcommand{\cupdot}{\mathbin{\mathaccent\cdot\cup}}
\DeclareMathOperator{\poly}{poly}
\newcommand{\OPT}{\texttt{OPT}}
\newcommand{\D}{\mathcal{D}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\A}{\mathcal{A}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\O}[1]{\mathcal{O}\left( #1\right) }
\newcommand{\Ot}[1]{\tilde{\mathcal{O}}\left( #1\right) }
\newcommand{\Om}[1]{\Omega\left( #1\right) }
\newcommand{\Omt}[1]{\tilde{\Omega}\left( #1\right) }
\newcommand{\Tt}[1]{\tilde{\Theta}\left( #1\right) }
\newcommand{\Th}[1]{{\Theta}\left( #1\right) }
\newcommand{\T}[2]{{\mathcal{U}}_{#1}\left( #2\right) }
\newcommand{\set}[1]{\left\{#1\right\}}

\newcommand{\singleedge}[1]{{\mathcal{L}}\left( #1\right) }
\newcommand{\singleedgep}[2]{{\mathcal{L}^{#2}}\left( #1\right) }


\begin{document}

\maketitle

%TODO mandatory: add short abstract of the document
\begin{abstract}
We consider the problem of finding an edge in a hidden undirected graph $G = (V, E)$ with $n$ vertices, in a model where we only allowed queries that ask whether or not a subset of vertices contains an edge. We study the non-adaptive model and show that while in the deterministic model the optimal algorithm requires $\binom{n}{2}$ queries (i.e., querying for any possible edge separately), in the randomized model $\Tt{n}$ queries are sufficient (and needed) in order to find an edge.\\
In addition, we study the query complexity for specific families of graphs, including Stars, Cliques, and Matchings, for both the randomized and deterministic models.\\
Lastly, for general graphs, we show a trade-off between the query complexity and the number of rounds, $r$, made by an adaptive algorithm. We present two algorithms with $\O{rn^{2/r}}$ and $\Ot{rn^{1/r}}$ sample complexity for the deterministic and randomized models, respectively.
\end{abstract}

\section{Introduction}\label{sec:intro}	
	\input{introduction}
	
\subsection{Our Results}
	\input{results}
\subsection{Paper's Structure}
	\input{structure}
	
\section{Context and Related Work}\label{sec:related}
	\input{related}
	
\section{Model and Preliminaries}\label{sec:model}	
	\input{prelim}
	
\section{Finding an Edge in a Hidden Graph}\label{sec:general}
    \input{general}
	
\section{Finding an Edge in Special Cases}\label{sec:special}	
	\input{special}
		
\section{Edge Finding Using $r$ Rounds}\label{sec:rounds}	
	\input{rounds}

\section{Discussion and Open Problems}\label{sec:discussion}	
	\input{discussion}


%%
%% Bibliography
%%

%% Please use bibtex, 

\bibliography{main}

\appendix
	\input{welfareOXS}	
	\input{appendix}	



\end{document}

